Understanding the Effects of Data Parallelism and Sparsity on Neural Network Training

We study two factors in neural network training: data parallelism and sparsity; here, data parallelism means processing training data in parallel using distributed systems (or equivalently increasing batch size), so that training can be accelerated; for sparsity, we refer to pruning parameters in a neural network model, so as to reduce computational and memory cost. Despite their promising benefits, however, understanding of their effects on neural network training remains elusive. In this work, we first measure these effects rigorously by conducting extensive experiments while tuning all metaparameters involved in the optimization. As a result, we find across various workloads of data set, network model, and optimization algorithm that there exists a general scaling trend between batch size and number of training steps to convergence for the effect of data parallelism, and further, difficulty of training under sparsity. Then, we develop a theoretical analysis based on the convergence properties of stochastic gradient methods and smoothness of the optimization landscape, which illustrates the observed phenomena precisely and generally, establishing a better account of the effects of data parallelism and sparsity on neural network training.

==> text/broaderimpact.tex <==
\section*{Broader Impact}

A fundamental aim of this research paper is linked to the idea of improving the efficiency of deep learning technologies by studying the general behaviors of sparse neural network models in regard to the effects of data scaling in their training.
Using large models has been a key to success in the development of highly intelligent systems in recent years, however, it often has limited accessibility, and thus simultaneously poses significant challenges to those who may not have enough computing resources to employ such models.
A part of our results indicates that neural networks in a compressed form can utilize given computing resources more effectively during training.
Hence, we believe that our study can potentially render a positive impact in the general computing research community without incentivizing a particular group of individuals.
Our results can also lead to a development of more efficient hardwares in new ways, which is believed to have a long-term benefit to society.
There could always be negative implications of scientific and technological advancements, however, it is our current belief that this work, being theoretical and focusing on understanding neural networks, is distant from having negative impacts or foreseeable potential risks in the near future.


==> text/developments.tex <==
\section{Developments}

%---------------------------------------------------------------------------------------------------
% MNIST
%---------------------------------------------------------------------------------------------------
%\begin{figure}[h]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=23mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-goal-error-0.02-ts-0.5}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-goal-error-0.02-ts-0.7}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/combinations/{simple-cnn-base-sgd-goal-error-0.02-var-sparsity}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/combinations/{simple-cnn-base-sgd-goal-error-0.02-var-sparsity-normalized}.eps}
%        \caption{SGD}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=23mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-goal-error-0.02-ts-0.5}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-goal-error-0.02-ts-0.7}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/combinations/{simple-cnn-base-momentum-goal-error-0.02-var-sparsity}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/combinations/{simple-cnn-base-momentum-goal-error-0.02-var-sparsity-normalized}.eps}
%        \caption{Momentum}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=23mm]{figure/s2r-bs/trends/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.0}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/trends/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.5}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/trends/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.7}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/trends/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.9}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/combinations/{simple-cnn-base-nesterov-goal-error-0.02-var-sparsity}.eps}
%        \includegraphics[height=23mm]{figure/s2r-bs/combinations/{simple-cnn-base-nesterov-goal-error-0.02-var-sparsity-normalized}.eps}
%        \caption{Nesterov}
%    \end{subfigure}
%    \caption{
%        Effect of \{sparsity\}.\\
%        mnist, simple-cnn-base, \{sgd, momentum, nesterov\}, constant, ge:0.02, ts: \{0.0, 0.5, 0.7, 0.9\}.
%    }
%    \label{fig:s2r-bs-mnist-all-optimizer}
%\end{figure}
%
%\begin{figure}[h]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{simple-cnn-base-goal-error-0.02-ts-0.0-var-optimizer}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{simple-cnn-base-goal-error-0.02-ts-0.5-var-optimizer}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{simple-cnn-base-goal-error-0.02-ts-0.7-var-optimizer}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{simple-cnn-base-goal-error-0.02-ts-0.9-var-optimizer}.eps}
%    \end{subfigure}
%    \caption{
%        Effect of \{optimizer\}.\\
%        mnist, simple-cnn-base, \{sgd, momentum, nesterov\}, constant, ge:0.02, ts: \{0.0, 0.5, 0.7, 0.9\}.
%    }
%    \label{fig:s2r-bs-mnist-compare-optimizers}
%\end{figure}
%
%\begin{figure}[h]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0-bs-4-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0-bs-32-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0-bs-256-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0-bs-2048-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0-bs-16384-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9-bs-4-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9-bs-32-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9-bs-256-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9-bs-2048-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9-bs-16384-lr}.eps}
%        \caption{SGD; learning rate}
%    \end{subfigure}
%    \caption{
%        Metaparameters for mnist experiments.
%        SGD.
%    }
%    \label{fig:s2r-metaparameters-mnist-sgd}
%\end{figure}
%
%\begin{figure}[h]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-4-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-32-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-256-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-2048-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-16384-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-4-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-32-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-256-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-2048-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-16384-lr}.eps}
%        \caption{Momentum; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-4-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-32-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-256-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-2048-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-16384-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-4-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-32-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-256-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-2048-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-16384-momentum}.eps}
%        \caption{Momentum; momentum}
%    \end{subfigure}
%    \caption{
%        Metaparameters for mnist experiments.
%        Momentum.
%    }
%    \label{fig:s2r-metaparameters-mnist-momentum}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.0-bs-4-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.0-bs-32-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.0-bs-256-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.0-bs-2048-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.0-bs-16384-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.9-bs-4-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.9-bs-32-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.9-bs-256-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.9-bs-2048-lr}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.9-bs-16384-lr}.eps}
%        \caption{Nesterov; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.0-bs-4-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.0-bs-32-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.0-bs-256-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.0-bs-2048-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.0-bs-16384-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.9-bs-4-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.9-bs-32-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.9-bs-256-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.9-bs-2048-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.9-bs-16384-momentum}.eps}
%        \caption{Nesterov; momentum}
%    \end{subfigure}
%    \caption{
%        Metaparameters for mnist experiments.
%        Nesterov.
%    }
%    \label{fig:s2r-metaparameters-mnist-nesterov}
%\end{figure}


%---------------------------------------------------------------------------------------------------
% Fashion MNIST
%---------------------------------------------------------------------------------------------------

% goal error 0.12
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.0}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.7}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.9}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-var-sparsity}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-var-sparsity-normalized}.eps}
%        \caption{SGD}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.0}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.7}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.9}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-var-sparsity}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-var-sparsity-normalized}.eps}
%        \caption{Momentum}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.12-ts-0.0}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.12-ts-0.7}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.12-ts-0.9}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.12-var-sparsity}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.12-var-sparsity-normalized}.eps}
%        \caption{Nesterov}
%    \end{subfigure}
%    \caption{
%        Effect of \{sparsity\}.\\
%        fmnist, simple-cnn-base, \{sgd, momentum, nesterov\}, constant, ge:0.12, ts: \{0.0, 0.7, 0.9\}.
%    }
%    \label{fig:s2r-bs-fmnist-ge-0.12-all-optimizer}
%\end{figure}

%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-constant-goal-error-0.12-ts-0.0-var-optimizer}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-constant-goal-error-0.12-ts-0.0-var-optimizer-normalized}.eps}
%        %\includegraphics[height=34mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-constant-goal-error-0.12-ts-0.7-var-optimizer}.eps}
%        %\includegraphics[height=34mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-constant-goal-error-0.12-ts-0.7-var-optimizer-normalized}.eps}\\
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-constant-goal-error-0.12-ts-0.9-var-optimizer}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-constant-goal-error-0.12-ts-0.9-var-optimizer-normalized}.eps}
%    \end{subfigure}
%    \caption{
%        Effect of \{optimizer\}.\\
%        fmnist, simple-cnn-base, \{sgd, momentum, nesterov\}, constant, ge:0.12, ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-bs-fmnist-ge-0.12-compare-optimizers}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.0-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.0-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.0-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.0-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.0-bs-16384-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.9-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.9-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.9-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.9-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.12-ts-0.9-bs-16384-learning_rate}.eps}
%        \caption{SGD; learning rate}
%    \end{subfigure}
%    \caption{
%        Metaparameters for fmnist (goal error 0.12) experiments.
%        SGD.
%    }
%    \label{fig:s2r-metaparameters-fmnist-ge-0.12-sgd}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.0-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.0-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.0-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.0-bs-2048-learning_rate}.eps}\\
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.0-bs-16384-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.9-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.9-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.9-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.9-bs-2048-learning_rate}.eps}
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.9-bs-16384-learning_rate}.eps}
%        \caption{Momentum; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.0-bs-4-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.0-bs-32-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.0-bs-256-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.0-bs-2048-momentum}.eps}\\
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.0-bs-16384-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.9-bs-4-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.9-bs-32-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.9-bs-256-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.9-bs-2048-momentum}.eps}
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.9-bs-16384-momentum}.eps}
%        \caption{Momentum; momentum}
%    \end{subfigure}
%    \caption{
%        Metaparameters for fmnist (goal error 0.12) experiments.
%        Momentum.
%    }
%    \label{fig:s2r-metaparameters-fmnist-ge-0.12-momentum}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-2048-learning_rate}.eps}\\
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-16384-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-2048-learning_rate}.eps}
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-16384-learning_rate}.eps}
%        \caption{Nesterov; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-4-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-32-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-256-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-2048-momentum}.eps}\\
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-16384-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-4-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-32-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-256-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-2048-momentum}.eps}
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-16384-momentum}.eps}
%        \caption{Nesterov; momentum}
%    \end{subfigure}
%    \caption{
%        Metaparameters for fmnist (goal error 0.12) experiments.
%        Nesterov.
%    }
%    \label{fig:s2r-metaparameters-fmnist-ge-0.12-nesterov}
%\end{figure}

%% goal error 0.14
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.0}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.7}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.9}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-var-sparsity}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-var-sparsity-normalized}.eps}
%        \caption{SGD}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.0}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.7}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.9}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-var-sparsity}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-var-sparsity-normalized}.eps}
%        \caption{Momentum}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.7}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-var-sparsity}.eps}
%        \includegraphics[height=27mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-var-sparsity-normalized}.eps}
%        \caption{Nesterov}
%    \end{subfigure}
%    \caption{
%        Effect of \{sparsity\}.\\
%        fmnist, simple-cnn-base, \{sgd, momentum, nesterov\}, constant, ge:0.14, ts: \{0.0, 0.7, 0.9\}.
%    }
%    \label{fig:s2r-bs-fmnist-all-optimizer}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-constant-goal-error-0.14-ts-0.0-var-optimizer}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-constant-goal-error-0.14-ts-0.0-var-optimizer-normalized}.eps}
%        %\includegraphics[height=34mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-constant-goal-error-0.14-ts-0.7-var-optimizer}.eps}
%        %\includegraphics[height=34mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-constant-goal-error-0.14-ts-0.7-var-optimizer-normalized}.eps}\\
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-constant-goal-error-0.14-ts-0.9-var-optimizer}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-constant-goal-error-0.14-ts-0.9-var-optimizer-normalized}.eps}
%    \end{subfigure}
%    \caption{
%        Effect of \{optimizer\}.\\
%        fmnist, simple-cnn-base, \{sgd, momentum, nesterov\}, constant, ge:0.14, ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-bs-fmnist-compare-optimizers}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.0-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.0-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.0-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.0-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.0-bs-16384-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.9-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.9-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.9-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.9-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-sgd-constant-goal-error-0.14-ts-0.9-bs-16384-learning_rate}.eps}
%        \caption{SGD; learning rate}
%    \end{subfigure}
%    \caption{
%        Metaparameters for fmnist experiments.
%        SGD.
%    }
%    \label{fig:s2r-metaparameters-fmnist-sgd}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.0-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.0-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.0-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.0-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.0-bs-16384-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.9-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.9-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.9-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.9-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.9-bs-16384-learning_rate}.eps}
%        \caption{Momentum; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.0-bs-4-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.0-bs-32-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.0-bs-256-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.0-bs-2048-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.0-bs-16384-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.9-bs-4-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.9-bs-32-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.9-bs-256-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.9-bs-2048-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.14-ts-0.9-bs-16384-momentum}.eps}
%        \caption{Momentum; momentum}
%    \end{subfigure}
%    \caption{
%        Metaparameters for fmnist experiments.
%        Momentum.
%    }
%    \label{fig:s2r-metaparameters-fmnist-momentum}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-16384-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-16384-learning_rate}.eps}
%        \caption{Nesterov; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-4-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-32-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-256-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-2048-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.0-bs-16384-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-4-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-32-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-256-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-2048-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{fmnist-simple-cnn-base-nesterov-constant-goal-error-0.14-ts-0.9-bs-16384-momentum}.eps}
%        \caption{Nesterov; momentum}
%    \end{subfigure}
%    \caption{
%        Metaparameters for fmnist experiments.
%        Nesterov.
%    }
%    \label{fig:s2r-metaparameters-fmnist-nesterov}
%\end{figure}



%---------------------------------------------------------------------------------------------------
% CIFAR
%---------------------------------------------------------------------------------------------------
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-var-sparsity}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-var-sparsity-normalized}.eps}
%        \caption{SGD}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-var-sparsity}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-var-sparsity-normalized}.eps}
%        \caption{Momentum}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-var-sparsity}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-var-sparsity-normalized}.eps}
%        \caption{Nesterov}
%    \end{subfigure}
%    \caption{
%        Effect of \{sparsity\}.\\
%        cifar-10, resnet-8-nobn, \{sgd, momentum, nesterov\}, linear, ge:0.4, ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-bs-cifar-all-optimizer}
%\end{figure}

%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-linear-goal-error-0.4-ts-0.0-var-optimizer}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-linear-goal-error-0.4-ts-0.0-var-optimizer-normalized}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-linear-goal-error-0.4-ts-0.9-var-optimizer}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-linear-goal-error-0.4-ts-0.9-var-optimizer-normalized}.eps}
%    \end{subfigure}
%    \caption{
%        Effect of \{optimizer\}.\\
%        cifar-10, resnet-8-nobn, \{sgd, momentum, nesterov\}, linear, ge:0.4, ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-bs-cifar-compare-optimizers}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-2048-learning_rate}.eps}\\
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-4096-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-2048-learning_rate}.eps}
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-4096-learning_rate}.eps}
%        \caption{SGD; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-4-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-32-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-256-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-2048-decay_steps}.eps}\\
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-4096-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-4-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-32-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-256-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-2048-decay_steps}.eps}
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-4096-decay_steps}.eps}
%        \caption{SGD; decay steps (T)}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-4-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-32-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-256-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-2048-end_learning_rate_factor}.eps}\\
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.0-bs-4096-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-4-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-32-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-256-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-2048-end_learning_rate_factor}.eps}
%        %\includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-sgd-linear-goal-error-0.4-ts-0.9-bs-4096-end_learning_rate_factor}.eps}
%        \caption{SGD; end learning rate factor ($\alpha$)}
%    \end{subfigure}
%    \caption{
%        Metaparameters for cifar-10 experiments.
%        SGD.
%    }
%    \label{fig:s2r-metaparameters-cifar-sgd}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-4096-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-4096-learning_rate}.eps}
%        \caption{Momentum; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-4096-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-4096-learning_rate}.eps}
%        \caption{Momentum; momentum}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-4-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-32-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-256-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-2048-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-4096-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-4-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-32-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-256-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-2048-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-4096-decay_steps}.eps}
%        \caption{Momentum; decay steps (T)}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-4-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-32-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-256-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-2048-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.0-bs-4096-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-4-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-32-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-256-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-2048-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-momentum-linear-goal-error-0.4-ts-0.9-bs-4096-end_learning_rate_factor}.eps}
%        \caption{Momentum; end learning rate factor ($\alpha$)}
%    \end{subfigure}
%    \caption{
%        Metaparameters for cifar-10 experiments.
%        Momentum.
%    }
%    \label{fig:s2r-metaparameters-cifar-momentum}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-4096-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-4096-learning_rate}.eps}
%        \caption{Nesterov; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-4096-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-4-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-32-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-256-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-2048-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-4096-learning_rate}.eps}
%        \caption{Nesterov; momentum}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-4-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-32-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-256-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-2048-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-4096-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-4-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-32-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-256-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-2048-decay_steps}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-4096-decay_steps}.eps}
%        \caption{Nesterov; decay steps (T)}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-4-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-32-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-256-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-2048-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0-bs-4096-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-4-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-32-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-256-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-2048-end_learning_rate_factor}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9-bs-4096-end_learning_rate_factor}.eps}
%        \caption{Nesterov; end learning rate factor ($\alpha$)}
%    \end{subfigure}
%    \caption{
%        Metaparameters for cifar-10 experiments.
%        Nesterov.
%    }
%    \label{fig:s2r-metaparameters-cifar-nesterov}
%\end{figure}


%---------------------------------------------------------------------------------------------------
% MNIST; Noise; metaparameter
%---------------------------------------------------------------------------------------------------
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.0}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.9}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-var-sparsity}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-var-sparsity-normalized}.eps}
%        \caption{SGD}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-var-sparsity}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-var-sparsity-normalized}.eps}
%        \caption{Momentum}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-var-sparsity}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-var-sparsity-normalized}.eps}
%        \caption{Nesterov}
%    \end{subfigure}
%    \caption{
%        Effect of \{sparsity\}.\\
%        mnist, simple-cnn-base, \{sgd, momentum, nesterov\}, constant, ge:0.02, noise, ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-bs-mnist-noise-all-optimizer}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{simple-cnn-base-constant-goal-error-0.02-noise-ts-0.0-var-optimizer}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{simple-cnn-base-constant-goal-error-0.02-noise-ts-0.0-var-optimizer-normalized}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{simple-cnn-base-constant-goal-error-0.02-noise-ts-0.9-var-optimizer}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{simple-cnn-base-constant-goal-error-0.02-noise-ts-0.9-var-optimizer-normalized}.eps}
%    \end{subfigure}
%    \caption{
%        Effect of \{optimizer\}.\\
%        mnist, simple-cnn-base, \{sgd, momentum, nesterov\}, constant, ge:0.02, noise, ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-bs-mnist-noise-compare-optimizers}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.0-bs-2-noise_scale}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.0-bs-16-noise_scale}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.0-bs-128-noise_scale}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.0-bs-1024-noise_scale}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.0-bs-4096-noise_scale}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.9-bs-2-noise_scale}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.9-bs-16-noise_scale}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.9-bs-128-noise_scale}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.9-bs-1024-noise_scale}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.9-bs-4096-noise_scale}.eps}
%        \caption{SGD; noise scale}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.0-bs-2-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.0-bs-16-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.0-bs-128-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.0-bs-1024-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.0-bs-4096-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.9-bs-2-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.9-bs-16-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.9-bs-128-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.9-bs-1024-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-ts-0.9-bs-4096-learning_rate}.eps}
%        \caption{SGD; learning rate}
%    \end{subfigure}
%    \caption{
%        Metaparameters for MSGD.\\
%        mnist, simple-cnn-base, sgd, constant, ge:0.02, noise (MSGD), ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-metaparameters-mnist-noise-sgd}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-2-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-16-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-128-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-1024-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-4096-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-2-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-16-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-128-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-1024-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-4096-noise_scale}.eps}
%        \caption{Momentum; noise scale}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-2-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-16-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-128-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-1024-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-4096-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-2-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-16-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-128-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-1024-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-4096-learning_rate}.eps}
%        \caption{Momentum; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-2-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-16-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-128-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-1024-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.0-bs-4096-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-2-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-16-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-128-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-1024-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-ts-0.9-bs-4096-momentum}.eps}
%        \caption{Momentum; momentum}
%    \end{subfigure}
%    \caption{
%        Metaparameters for MSGD.\\
%        mnist, simple-cnn-base, momentum, constant, ge:0.02, noise (MSGD), ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-metaparameters-mnist-noise-momentum}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-2-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-16-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-128-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-1024-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-4096-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-2-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-16-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-128-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-1024-noise_scale}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-4096-noise_scale}.eps}
%        \caption{Nesterov; noise scale}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-2-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-16-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-128-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-1024-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-4096-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-2-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-16-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-128-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-1024-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-4096-learning_rate}.eps}
%        \caption{Nesterov; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-2-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-16-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-128-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-1024-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.0-bs-4096-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-2-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-16-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-128-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-1024-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-ts-0.9-bs-4096-momentum}.eps}
%        \caption{Nesterov; momentum}
%    \end{subfigure}
%    \caption{
%        Metaparameters for MSGD.\\
%        mnist, simple-cnn-base, nesterov, constant, ge:0.02, noise (MSGD), ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-metaparameters-mnist-noise-nesterov}
%\end{figure}
%
%%---------------------------------------------------------------------------------------------------
%% MNIST; Noise; fixed 0.01
%%---------------------------------------------------------------------------------------------------
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-ts-0.0}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-ts-0.9}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-var-sparsity}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-var-sparsity-normalized}.eps}
%        \caption{SGD}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.0}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.9}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-var-sparsity}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-var-sparsity-normalized}.eps}
%        \caption{Momentum}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.0}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.9}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-var-sparsity}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-var-sparsity-normalized}.eps}
%        \caption{Nesterov}
%    \end{subfigure}
%    \caption{
%        Effect of \{sparsity\}.\\
%        mnist, simple-cnn-base, \{sgd, momentum, nesterov\}, constant, ge:0.02, noise (fixed 0.01), ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-bs-mnist-noise-0.01-all-optimizer}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{simple-cnn-base-constant-goal-error-0.02-noise-0.01-ts-0.0-var-optimizer}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{simple-cnn-base-constant-goal-error-0.02-noise-0.01-ts-0.0-var-optimizer-normalized}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{simple-cnn-base-constant-goal-error-0.02-noise-0.01-ts-0.9-var-optimizer}.eps}
%        \includegraphics[height=34mm]{figure/s2r-bs/combinations/{simple-cnn-base-constant-goal-error-0.02-noise-0.01-ts-0.9-var-optimizer-normalized}.eps}
%    \end{subfigure}
%    \caption{
%        Effect of \{optimizer\}.\\
%        mnist, simple-cnn-base, \{sgd, momentum, nesterov\}, constant, ge:0.02, noise (fixed 0.01), ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-bs-mnist-noise-0.01-compare-optimizers}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-2-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-16-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-128-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-1024-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-4096-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-2-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-16-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-128-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-1024-learning_rate}.eps}
%        \includegraphics[height=27mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-4096-learning_rate}.eps}
%        \caption{SGD; learning rate}
%    \end{subfigure}
%    \caption{
%        Metaparameters for MSGD.\\
%        mnist, simple-cnn-base, sgd, constant, ge:0.02, noise (MSGD; fixed 0.01), ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-metaparameters-mnist-noise-0.01-sgd}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-2-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-16-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-128-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-1024-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-4096-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-2-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-16-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-128-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-1024-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-4096-learning_rate}.eps}
%        \caption{Momentum; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-2-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-16-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-128-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-1024-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-4096-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-2-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-16-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-128-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-1024-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-momentum-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-4096-momentum}.eps}
%        \caption{Momentum; momentum}
%    \end{subfigure}
%    \caption{
%        Metaparameters for MSGD.\\
%        mnist, simple-cnn-base, momentum, constant, ge:0.02, noise (MSGD; fixed 0.01), ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-metaparameters-mnist-noise-0.01-momentum}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-2-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-16-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-128-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-1024-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-4096-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-2-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-16-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-128-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-1024-learning_rate}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-4096-learning_rate}.eps}
%        \caption{Nesterov; learning rate}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-2-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-16-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-128-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-1024-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.0-bs-4096-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-2-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-16-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-128-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-1024-momentum}.eps}
%        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-nesterov-constant-goal-error-0.02-noise-0.01-ts-0.9-bs-4096-momentum}.eps}
%        \caption{Nesterov; momentum}
%    \end{subfigure}
%    \caption{
%        Metaparameters for MSGD.\\
%        mnist, simple-cnn-base, nesterov, constant, ge:0.02, noise (MSGD; fixed 0.01), ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-metaparameters-mnist-noise-0.01-nesterov}
%\end{figure}
%
%
%
%%---------------------------------------------------------------------------------------------------
%% Combinations
%%---------------------------------------------------------------------------------------------------
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-sgd-constant-goal-error-0.02-ts-var-noise-effect}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-sgd-constant-goal-error-0.02-ts-var-noise-effect-normalized}.eps}
%        \caption{SGD}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-momentum-constant-goal-error-0.02-ts-var-noise-effect}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-momentum-constant-goal-error-0.02-ts-var-noise-effect-normalized}.eps}
%        \caption{Momentum}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-nesterov-constant-goal-error-0.02-ts-var-noise-effect}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-nesterov-constant-goal-error-0.02-ts-var-noise-effect-normalized}.eps}
%        \caption{Nesterov}
%    \end{subfigure}
%    \caption{
%        Effect of \{noise (MSGD) and sparsity\}.\\
%        mnist, simple-cnn-base, \{sgd, momentum, nesterov\}, constant, ge:0.02, noise: No or Yes (MSGD), ts: \{0.0, 0.9\}.
%    }
%    \label{fig:s2r-bs-mnist-noise-effect-all-optimizer}
%\end{figure}







==> text/experiments.tex <==
%\section{Experiments}
%\section{The effects of data parallelism and sparsity in training neural networks}
\vspace{-2mm}
\section{Measuring the effects of data parallelism and sparsity}
\vspace{-2.6mm}


%--------------------------------------------------------------------------------------------------
\subsection{Setup}
\vspace{-2.6mm}

\textbf{Experiment protocol}.\quad
We closely follow the experiment settings in~\cite{shallue2018measuring}.
For a given workload (\ie, data set, model, optimization algorithm) and study (\ie, batch size, sparsity level), we measure the number of training steps to reach a pre-defined goal error (\eg, error rate for image classification).
In this process, we search for the best metaparameters with a budget of runs to record the lowest number of steps, namely \emph{steps-to-result}, as our primary quantity of interest.
For each run of training, we evaluate the intermediate model checkpoints on the entire validation set of a given data set at every fixed iterations to check if they reached the goal error.
We describe more details and the scale of our experiments in Appendix~\ref{sec:expscale}.

\textbf{Workloads}.\quad
We consider the workloads constructed as the combinations of the following data sets, models, and optimization algorithms:
(data sets) MNIST, Fashion-MNIST, CIFAR-10;
(models) Simple-CNN, ResNet-8;
(optimization algorithms) SGD, Momentum, Nesterov with either a constant learning rate or a linear learning rate decay schedule.
In the main paper, we present results for the following four workloads:
(W1) MNIST, Simple-CNN, SGD with a constant learning rate,
(W2) MNIST, Simple-CNN, Momentum with a constant learning rate,
(W3) Fashion-MNIST, Simple-CNN, Momentum with a constant learning rate, and
(W4) CIFAR-10, ResNet-8, Nesterov with a linear learning rate decay;
results for other workloads of combinations of above are provided in Appendix~\ref{sec:additional}.
%other results for workloads of the combinations of above are provided in Appendices~\ref{sec:edp} and~\ref{sec:mparams}.
We use $10$\% of the training set as a validation set, and the goal validation errors are set to be $0.02$, $0.12$, $0.4$ for MNIST, Fashion-MNIST, CIFAR-10, respectively.
The network models are the same as~\citep{shallue2018measuring}, except that we remove dropout to prevent any effect on sparsification.

\textbf{Metaparameter search}.\quad
We perform a quasi-random search to tune metaparameters efficiently.
More precisely, we first generate Sobol low-discrepancy sequences in a unit hypercube and convert them into metaparameters of interest, while taking into account a predefined search space for each metaparameter.
The generated values for each metaparameter is in length of the budget of trials, and the search space is designed based on preliminary experimental results.

\textbf{Pruning}.\quad
We use the connection sensitivity saliency criterion in~\cite{lee2018snip} to prune a given network model at initialization prior to training.
Sparse neural networks can be obtained by many different ways, and yet, for the purpose of this work, they must not undergo any training beforehand so we can measure the effects of data parallelism in isolation on training neural networks from scratch.

%\textbf{Experiment protocol}.\quad
%We closely follow the experiment protocol presented in~\cite{shallue2018measuring}.
%For each study (\ie, batch size, sparsity level) and workload (\ie, data set, model, optimization algorithm), we measure the number of training steps to achieve a goal validation error, or \emph{steps-to-result}, as the primary quantity of interest.
%For each study on a workload, we record the lowest steps-to-result while searching the best metaparameters within a budget of trials of 100 runs.
%For each run, we check the error on the entire examples in a validation set at every 16 steps.

%\textbf{Workloads}.\quad
%We consider the following workloads of \{data set, model, optimization algorithm\}:
%(W1) Simple-CNN on MNIST trained using SGD optimizer with a constant learning rate;
%(W2) Simple-CNN on MNIST trained using SGD with momentum (Momentum) or Nesterov momentum (Nesterov) optimizer with a constant learning rate;
%(W3) ResNet-8 on CIFAR-10 trained using the Nesterov optimizer with a linear learning rate decay schedule.
%All metaparameters involved in these workloads (\ie, learning rate, momentum, decay steps and decay factor) are tuned independently for each study by a quasi-random search.
%The goal validation errors are set to be 0.02 and 0.4 for W1/W2 and W3, respectively.
%We remove dropout in Simple-CNN to avoid any effect on sparsification.
%We refer to~\cite{shallue2018measuring} for further architecture details.

%\textbf{Metaparameter search}.\quad
%We perform a quasi-random search to tune metaparameters efficiently.
%Specifically, we first generate Sobol low-discrepancy sequences in a unit hypercube and convert them into metaparameters of interest, while taking into account a predefined search space for each metaparameter.
%The generated values for each metaparameter is length of the budget of trials (\ie, 100) for all studies, and the search space is designed based on preliminary experimental results.

%\textbf{Pruning}.\quad
%Sparse neural networks can be obtained by many different ways, and yet, for the purpose of this work, they must not undergo any training so we can measure the effects of data parallelism on training sparse neural networks in isolation. %while training from scratch.
%Adopting the connection sensitivity saliency criterion suggested in~\cite{lee2018snip}, we prune a given network at initialization and train the resulting sparse neural network from scratch.



%--------------------------------------------------------------------------------------------------
%\subsection{Results: data parallelism in training sparse neural networks}
\subsection{Results}
\vspace{-3mm}

% Main results
\begin{figure}[h!]
    \centering
    \begin{subfigure}{.9998\textwidth}
        \centering
        \includegraphics[height=33mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0}.eps}
        \includegraphics[height=33mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9}.eps}
        \includegraphics[height=33mm]{figure/s2r-bs/combinations/{simple-cnn-base-sgd-goal-error-0.02-var-sparsity}.eps}
        \includegraphics[height=33mm]{figure/s2r-bs/combinations/{simple-cnn-base-sgd-goal-error-0.02-var-sparsity-normalized}.eps}
        \caption{MNIST, Simple-CNN, SGD}
    \end{subfigure}
    \begin{subfigure}{.9998\textwidth}
        \centering
        \includegraphics[height=33mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0}.eps}
        \includegraphics[height=33mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9}.eps}
        \includegraphics[height=33mm]{figure/s2r-bs/combinations/{simple-cnn-base-momentum-goal-error-0.02-var-sparsity}.eps}
        \includegraphics[height=33mm]{figure/s2r-bs/combinations/{simple-cnn-base-momentum-goal-error-0.02-var-sparsity-normalized}.eps}
        \caption{MNIST, Simple-CNN, Momentum}
    \end{subfigure}
    \begin{subfigure}{.9998\textwidth}
        \centering
        \includegraphics[height=33mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.0}.eps}
        \includegraphics[height=33mm]{figure/s2r-bs/trends/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-ts-0.9}.eps}
        \includegraphics[height=33mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-var-sparsity}.eps}
        \includegraphics[height=33mm]{figure/s2r-bs/combinations/{fmnist-simple-cnn-base-momentum-constant-goal-error-0.12-var-sparsity-normalized}.eps}
        \caption{Fashion-MNIST, Simple-CNN, Momentum}
    \end{subfigure}
    \begin{subfigure}{.9998\textwidth}
        \centering
        \includegraphics[height=33mm]{figure/s2r-bs/trends/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0}.eps}
        \includegraphics[height=33mm]{figure/s2r-bs/trends/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9}.eps}
        \includegraphics[height=33mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-var-sparsity}.eps}
        \includegraphics[height=33mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-var-sparsity-normalized}.eps}
        \caption{CIFAR-10, ResNet-8, Nesterov}
    \end{subfigure}
    \caption{
        The effects of data parallelism and sparsity on neural network training for various workloads.
        Across all workloads and sparsity levels, the same scaling pattern is observed for the relationship between batch size and steps-to-result: it starts with the initial phase of \emph{linear scaling} where increasing the batch size decreases the steps required to achieve the goal error inverse proportionally, and then there begins a region of \emph{diminishing returns}, which is followed by the saturating phase of \emph{maximal data parallelism} where increasing the batch size no longer speeds up the training process.
        Also, the effect of data parallelism in training sparse neural networks is no worse than that the dense, over-parameterized counterpart, despite the general difficulty of training sparse neural networks.
        %When training using a momentum based SGD (\eg, Momentum, Nesterov), the breakdown of the linear scaling regime often occurs much later at larger batch sizes for a network with higher sparsity; \ie, a \emph{critical batch size} can be even larger when training sparse neural networks.\mj{yes and you could even say that the effect of momentum (as by shifting the breakdown point) is significantly later? }
        %\mj{also this result section 2.2 is quite a wall of text and thus might be a bit hard to navigate (except careful sequential reading) if readers want to skip to particular aspects. want to maybe highlight/bolden particular keywords such as effect of momentum, sparsity etc}
        When training using a \emph{momentum} based SGD (\eg, Momentum, Nesterov), the breakdown of the linear scaling regime often occurs much later at larger batch sizes for a network with higher sparsity; \ie, a \emph{critical batch size} can be even larger when training sparse neural networks with momentum.
        For example, in the case of workload \{MNIST, Simple-CNN, Momentum\}, the critical batch size for the sparsity 90\% network is around $2^{11}$ whereas it is $2^{9}$ for the sparsity 0\% network (see the 4th column in row (b)).
        %The effect of momentum on increasing critical batch size can be seen further in Figure~\ref{fig:edp-optimizer}.
        This potentially indicates that one can exploit large batch sizes more effectively when training sparse neural networks than densely parameterized neural networks.
        We supply more results in Appendix~\ref{sec:additional}.
    }
    \label{fig:edp-main}
\end{figure}


% Comparing optimizers
\begin{figure}[t]
    \centering
    \begin{subfigure}{.9998\textwidth}
        \centering
        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-goal-error-0.02-ts-0.0-var-optimizer}.eps}
        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-goal-error-0.02-ts-0.5-var-optimizer}.eps}
        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-goal-error-0.02-ts-0.7-var-optimizer}.eps}
        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-goal-error-0.02-ts-0.9-var-optimizer}.eps}
    \end{subfigure}
    \caption{
        Comparing different optimization algorithms (SGD, Momentum, Nesterov) for the effects of data parallelism and sparsity.
        Across all sparsity levels, momentum based SGD optimizers (\ie, Momentum, Nesterov) record lower steps-to-result in a large batch regime and have much bigger critical batch sizes than SGD without momentum.
        Identifying such patterns is crucial especially when training in resource constrained environments, as practitioners can potentially benefit from reducing the training time by deciding a critical batch size properly, while utilizing resources more effectively.
    }
    \label{fig:edp-optimizer}
\end{figure}



%\begin{figure}[t]
%    %\vspace{-6mm}
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=28mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0}.eps}
%        \includegraphics[height=28mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-goal-error-0.02-ts-0.7}.eps}
%        \includegraphics[height=28mm]{figure/s2r-bs/trends/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9}.eps}
%        \includegraphics[height=28mm]{figure/s2r-bs/combinations/{simple-cnn-base-sgd-goal-error-0.02-var-sparsity}.eps}
%        \includegraphics[height=28mm]{figure/s2r-bs/combinations/{simple-cnn-base-sgd-goal-error-0.02-var-sparsity-normalized}.eps}
%        \caption{SGD}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=28mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0}.eps}
%        \includegraphics[height=28mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-goal-error-0.02-ts-0.7}.eps}
%        \includegraphics[height=28mm]{figure/s2r-bs/trends/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9}.eps}
%        \includegraphics[height=28mm]{figure/s2r-bs/combinations/{simple-cnn-base-momentum-goal-error-0.02-var-sparsity}.eps}
%        \includegraphics[height=28mm]{figure/s2r-bs/combinations/{simple-cnn-base-momentum-goal-error-0.02-var-sparsity-normalized}.eps}
%        \caption{Momentum}
%    \end{subfigure}
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=28mm]{figure/s2r-bs/trends/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.0}.eps}
%        \includegraphics[height=28mm]{figure/s2r-bs/trends/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.7}.eps}
%        \includegraphics[height=28mm]{figure/s2r-bs/trends/{simple-cnn-base-nesterov-goal-error-0.02-ts-0.9}.eps}
%        \includegraphics[height=28mm]{figure/s2r-bs/combinations/{simple-cnn-base-nesterov-goal-error-0.02-var-sparsity}.eps}
%        \includegraphics[height=28mm]{figure/s2r-bs/combinations/{simple-cnn-base-nesterov-goal-error-0.02-var-sparsity-normalized}.eps}
%        \caption{Nesterov}
%    \end{subfigure}
%    \caption{
%        Results of measuring the data parallelism in sparse neural network training using Simple-CNN on MNIST.
%        We first prune the network for \{0, 50, 70, 90\}\% sparsity levels, train using either SGD, SGD with momentum (Momentum), or SGD with Nesterov momentum (Nesterov) optimizer, and then record steps-to-result to achieve the goal error of 0.02.
%        Across all sparsity levels and optimizers, the same scaling pattern is observed for the relationship between batch size and steps-to-result: increasing the batch size initially decreases the steps required to achieve the goal error proportionally (\emph{linear scaling}), and then there begins a region of \emph{diminishing returns}, followed by the phase of \emph{maximal data parallelism} where increasing the batch size no longer speeds up the training.
%        Notably, the data parallelism in sparse neural network training is no worse than regular neural network training, despite the general difficulty of training sparse networks.
%        More interestingly, when training with momentum, the breakdown of the linear scaling regime occurs much later at larger batch sizes for a higher sparsity network; \ie, a \emph{critical batch size} can be even larger when training sparse neural networks (\eg, $2^{11}$ for the sparsity 90\% network compared to $2^{9}$ for the sparsity 0\% network when using Momentum).
%        This potentially indicates that one can exploit large batch sizes more effectively when training sparse neural networks than regular neural networks.
%    }
%    %\vspace{-2mm}
%    \label{fig:s2r-bs-mnist}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-goal-error-0.02-ts-0.0-var-optimizer}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-goal-error-0.02-ts-0.5-var-optimizer}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-goal-error-0.02-ts-0.7-var-optimizer}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{simple-cnn-base-goal-error-0.02-ts-0.9-var-optimizer}.eps}
%    \end{subfigure}
%    \caption{
%        Comparing the relationship between batch size and steps-to-result by different optimizers.
%        For all sparsity levels, Momentum and Nesterov optimizers are able to exploit much larger batch sizes than the plain SGD optimizer.
%        Identifying such pattern is crucial especially when training in resource constrained enviroments, as practitioners can benefit from reducing the training time by deciding a critical batch size properly, while utilizing resources more effectively.
%    }
%    \label{fig:s2r-bs-mnist-optimizer}
%\end{figure}

%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.0}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/trends/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-ts-0.9}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-var-sparsity}.eps}
%        \includegraphics[height=32mm]{figure/s2r-bs/combinations/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-var-sparsity-normalized}.eps}
%    \end{subfigure}
%    \caption{
%        Results of measuring the data parallelism in sparse neural network training using ResNet-8 on CIFAR-10.
%        We prune the network for \{0, 90\}\% sparsity levels, train using Nesterov optimizer with linear learning rate decay, and then record steps-to-result to achieve the goal error of 0.4.
%        A scaling pattern of data parallelism observed here is similar to that of the previous workloads; \ie, a critical batch size for the sparse network appears to be larger than that for the dense network.
%    }
%    \label{fig:s2r-bs-cifar}
%\end{figure}


First of all, we observe in each and every sparsity level across different workloads a general trend in the relationship between batch size and steps-to-result for the effects of data parallelism (see the 1st and 2nd columns in Figure~\ref{fig:edp-main}):
Initially, we observe a period of \emph{linear scaling} where doubling the batch size reduces the steps to achieve the goal error by half (\ie, it aligns closely with the dashed line), followed by a region of \emph{diminishing returns} where the reduction in the required number of steps by increasing the batch size is less than the inverse proportional amount (\ie, it starts to digress from the linear scaling region), which eventually arrives at a \emph{maximal data parallelism} (\ie, it hits a plateau) where increasing the batch size no longer decreases the steps to reach a goal error.
This is observed across other workloads of different combinations of data set, network model, and optimization algorithm as well as different goal errors (see Appendix~\ref{sec:additional}).
We note that our observation is consistent with the results of regular network training presented in~\citep{shallue2018measuring}.
%We develop theoretical insights based on convergence properties into this seemingly universal phenomenon in Section~\ref{sec:convergence}.
We develop a theory of the effect of data parallelism that precisely accounts for this universal phenomenon in Section~\ref{sec:convergence}.

When we put the results for all sparsity levels together, the effect of data parallelism can be clearly visible and compared (see the 3rd column in Figure~\ref{fig:edp-main}).
In general, we find that the higher the sparsity level, the longer it takes for a sparse network to reach the given goal error.
More precisely, a data parallelism curve for higher sparsity usually lies above than that for lower sparsity.
%For example, compared to the case of sparsity $0$\% (\ie, the dense, over-parameterized network), $90$\% sparse network takes about $2^{1.5}$ times longer training time (or the number of training steps), consistently across different batch sizes until each sparsity case hits its own region of diminishing returns.
%For example, compared to the case of sparsity $0$\% (\ie, the dense, over-parameterized network), $90$\% sparse network takes about $2^{1.5}$ times longer training time (or the number of training steps), consistently across different batch sizes (see Figure~\ref{fig:edp-ratio} in Appendix~\ref{sec:moreedp} for more precise comparison).
For example, compared to the case of sparsity $0$\% (\ie, the dense, over-parameterized network), $90$\% sparse network takes about $2-4$ times longer training time (or the number of training steps), consistently across different batch sizes (we provide more precise comparisons in Figure~\ref{fig:edp-ratio}, Appendix~\ref{sec:moreedp}).
Recall that we tune all metaparameters independently for each and every study case of batch size and sparsity level without relying on a single predefined training rule, so as to find the best steps-to-result.
Therefore, this result on the one hand corroborates the general difficulty of training sparse neural networks against the ease of training overly parameterized neural networks.
%We conduct theoretical analysis for this difficulty in Section~\ref{sec:lipschitz}.
%We further explain what may cause this difficulty based on our theory and a Lipschitz smoothness analysis in Section~\ref{sec:lipschitz}.
We further find a potential cause of this difficulty based on our theory and a Lipschitz smoothness analysis in Section~\ref{sec:lipschitz}.

On the other hand, when we normalize the y-axis of each plot by dividing by the number of steps for the first batch size, we can see the phase transitions more clearly.
As a result, we find that the regions of diminishing returns and maximal data parallelism appear no earlier when training sparse networks than the dense network (see the 4th column in Figure~\ref{fig:edp-main}).
This is quite surprising in that one could have easily guessed that the general optimization difficulty incurred by sparsification may influence the data parallelism too, at least to some degree; however, it turns out that the effects of data parallelism on sparse network training remain no worse than the dense case.
Moreover, notice that in many cases the breakdown of linear scaling regime occurs even much later at larger batch sizes for a higher sparsity case; this is especially evident for Momentum and Nesterov optimizers (\eg, compare training $90$\% sparse network using Momentum against $0$\% dense network).
In other words, for sparse networks, a \emph{critical batch size} can be larger, and hence, when it comes to training sparse neural networks, one can increase the batch size (or design a parallel computing system for distributed optimization) more effectively, while better exploiting given resources.
We find this result particularly promising since SGD with momentum is often the method of choice in practice.
We further show that momentum optimizers being capable of exploiting large batch sizes hold the same across different sparsity levels by displaying all plots together in Figure~\ref{fig:edp-optimizer}.
Overall, we believe that it is positively important to confirm the robustness of the data parallelism in sparse neural network training, which has been unknown thus far and difficult to estimate a priori.



%--------------------------------------------------------------------------------------------------
\subsection{Metaparameter search}

\begin{figure}[t]
    \centering
    \begin{subfigure}{.9998\textwidth}
        \centering
        \includegraphics[height=32mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-16}.eps}
        \includegraphics[height=32mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-128}.eps}
        \includegraphics[height=32mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-1024}.eps}
        \includegraphics[height=32mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-8192}.eps}\\
        \includegraphics[height=32mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-16}.eps}
        \includegraphics[height=32mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-128}.eps}
        \includegraphics[height=32mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-1024}.eps}
        \includegraphics[height=32mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-8192}.eps}
    \end{subfigure}
    \caption{
        Visualizing all trials (100) for Simple-CNN on MNIST trained using Momentum optimizer with a constant learning rate.
        Sparsity level (S) and batch size (B) are denoted at the top of each plot.
        The best trial that records the lowest steps-to-result is marked by gold star (\textcolor{Dandelion}{$\star$}).
        Complete/incomplete refer to the trials of goal reached/not reached given a maximum training step budget, while infeasible refers to the trial of divergence during training.
    }
    \label{fig:mparams-mnist-momentum}
\end{figure}


\begin{figure}[t]
    \centering
    \begin{subfigure}{.9998\textwidth}
        \centering
        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0-bs-4-lr}.eps}
        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0-bs-32-lr}.eps}
        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0-bs-256-lr}.eps}
        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0-bs-2048-lr}.eps}
        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.0-bs-16384-lr}.eps}
        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9-bs-4-lr}.eps}
        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9-bs-32-lr}.eps}
        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9-bs-256-lr}.eps}
        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9-bs-2048-lr}.eps}
        \includegraphics[height=26mm]{figure/s2r-metaparameters/{simple-cnn-base-sgd-goal-error-0.02-ts-0.9-bs-16384-lr}.eps}
    \end{subfigure}
    \caption{
        Visualizing metaparameter search results for the workload of \{MNIST, Simple-CNN, SGD\}.
        The metaparameter being tuned is the learning rate $\bar{\eta}$.
        We present results for different batch sizes ($2^2$, $2^5$, $2^8$, $2^{11}$, $2^{14}$ -- columns) and sparsity levels ($0$, $90$\% -- rows).
        The blue circles (\tikzcircle[MidnightBlue, fill=blue]{1.5pt}) denote successful runs (\ie, it reached the goal error), and the best trial that records the \emph{lowest} steps to reach the goal (\ie, steps-to-result) is marked by gold star (\textcolor{Dandelion}{$\star$}); also, the grey triangles (\textcolor{Gray}{$\blacktriangle$}) and red crosses (\textcolor{Red}{$\times$}) refer to incomplete and infeasible runs, respectively.
        We supply more results in Appendix~\ref{sec:moremparams}.
    }
    \label{fig:mparams-mnist-sgd}
    \vspace{-4mm}
\end{figure}

%\begin{figure}[t]
%    \centering
%    \begin{subfigure}{.9998\textwidth}
%        \centering
%        \includegraphics[height=30mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-16}.eps}
%        \includegraphics[height=30mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-128}.eps}
%        \includegraphics[height=30mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-1024}.eps}
%        \includegraphics[height=30mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.0-bs-8192}.eps}\\
%        \includegraphics[height=30mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-16}.eps}
%        \includegraphics[height=30mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-128}.eps}
%        \includegraphics[height=30mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-1024}.eps}
%        \includegraphics[height=30mm]{figure/complete-incomplete-infeasible/individual/{simple-cnn-base-momentum-goal-error-0.02-ts-0.9-bs-8192}.eps}
%    \end{subfigure}
%    \caption{
%        Visualizing all trials (100) for Simple-CNN on MNIST trained using Momentum optimizer with a constant learning rate.
%        Sparsity level (S) and batch size (B) are denoted at the top of each plot.
%        The best trial that records the lowest steps-to-result is marked by gold star (\textcolor{Dandelion}{$\star$}).
%        Complete/incomplete refer to the trials of goal reached/not reached given a maximum training step budget, while infeasible refers to the trial of divergence during training.
%    }
%    \label{fig:trials-momentum}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-learning_rate-ts-0.0-bs-16}.eps}
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-learning_rate-ts-0.9-bs-16}.eps}
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-learning_rate-ts-0.0-bs-1024}.eps}
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-learning_rate-ts-0.9-bs-1024}.eps}\\
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-momentum-ts-0.0-bs-16}.eps}
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-momentum-ts-0.9-bs-16}.eps}
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-momentum-ts-0.0-bs-1024}.eps}
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-momentum-ts-0.9-bs-1024}.eps}\\
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-decay_steps-ts-0.0-bs-16}.eps}
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-decay_steps-ts-0.9-bs-16}.eps}
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-decay_steps-ts-0.0-bs-1024}.eps}
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-decay_steps-ts-0.9-bs-1024}.eps}\\
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-end_learning_rate_factor-ts-0.0-bs-16}.eps}
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-end_learning_rate_factor-ts-0.9-bs-16}.eps}
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-end_learning_rate_factor-ts-0.0-bs-1024}.eps}
%    \includegraphics[height=30mm]{figure/validate-search-space/individual/{resnet8-v2-a-nobn-nesterov-linear-goal-error-0.4-end_learning_rate_factor-ts-0.9-bs-1024}.eps}\\
%    \caption{
%        Visualizing the metaparameter search results for ResNet-8 on CIFAR-10 trained using the Nesterov optimizer with a linear learning rate decay schedule.
%        Sparsity level (S) and batch size (B) are denoted at the top of each plot.
%        The best trial that records the lowest steps-to-result is marked by gold star (\textcolor{Dandelion}{$\star$}).
%    }
%    \label{fig:validate-search-space}
%\end{figure}


We perform metaparameter search to find the best metaparameter values that yield steps-to-result.
In this section, we present and analyze the metaparameter search results used to measure the effects of data parallelism studied in the previous section.
Specifically, we investigate the case of workload \{MNIST, Simple-CNN, Momentum\} where there are two metaparameters to tune (\ie, learning rate and momentum) as this allows us to analyze all metaparameters easily in one figure.
The results are presented in Figure~\ref{fig:mparams-mnist-momentum}, and other results can be found in Appendix~\ref{sec:moremparams}.

First of all, our quasi-random search enables us to sample metaparameters efficiently, so that they are distributed evenly (without being cluttered) in a log-space and flexibly (rather than sitting in a grid with fixed spacing) within the search spaces.
The search spaces are determined based on preliminary experiments and considered to be designed reasonably, in that the best metaparameters to yield lowest steps (marked by gold star \textcolor{Dandelion}{$\star$}) are located in the middle of the search ranges rather than sitting at the search boundaries, across different batch sizes and sparsity levels; \eg, the best learning rate is located around $10^{-2}$ while the best momentum is found around a bit larger than $0.9$.
Also, the best learning rate increases with batch size, which aligns well with the classic result in learning theory that large batch training allows using bigger learning rates.

Interestingly, there are two distinguished regions (\ie, complete (\tikzcircle[MidnightBlue, fill=blue]{1.5pt}) and incomplete (\textcolor{Gray}{$\blacktriangle$})) being separated by a seemingly linear boundary as per the relationship between learning rate and momentum.
This indicates that the optimization is being done by an interplay between these two metaparameters.
More precisely, if one metaparameter is not chosen carefully with respect to the other (\eg, increasing the learning rate for a fixed momentum), the optimizer may be stuck in a region spending time oscillating and eventually results in incomplete runs that did not reach a goal error within the maximum training iterations.
Also, we can see that the successful region (filled with blue circles \tikzcircle[MidnightBlue, fill=blue]{1.5pt}) becomes larger as with increasing batch size, showing that large batch training reaches a given goal error in less number of iterations than small batch training, and hence, yields more complete runs.

%We further present results for the workload \{MNIST, Simple-CNN, SGD\} in Figure~\ref{fig:mparams-mnist-sgd}.
%By isolating learning rate from momentum, it facilitates the search result analysis, and allows us to study the effect of sparsity theoretically.
%We will analyze this case based on convergence theory later in Section~\ref{sec:lipschitz}.

We further present results for the workload \{MNIST, Simple-CNN, SGD\} in Figure~\ref{fig:mparams-mnist-sgd}.
By isolating learning rate from momentum, it facilitates the search result analysis, and also allows us to study the effect of sparsity theoretically.
More specifically, notice that for each batch size, the size of the range for successful learning rate $\bar{\eta}$ decreases by introducing sparsity.
This supports our claim later in Section~\ref{sec:lipschitz} that sparsity reduces the smoothness of gradients.
We explain further in Appendix~\ref{sec:morelipschitz}.


==> text/relatedwork.tex <==
\section{Related work}

\textbf{data parallelism, batch science, large-batch training}.\quad

\textbf{compression and optimization of neural networks; pruning and training}.\quad

